Robust and Scalable Model Editing for Large Language Models

Large language models (LLMs) can make predictions using parametric knowledge--knowledge encoded in the model weights--or contextual knowledge--knowledge presented in the context. In many scenarios, a desirable behavior is that LLMs give precedence to contextual knowledge when it conflicts with the parametric knowledge, and fall back to using their parametric knowledge when the context is irrelevant. This enables updating and correcting the model's knowledge by in-context editing instead of retraining. Previous works have shown that LLMs are inclined to ignore contextual knowledge and fail to reliably fall back to parametric knowledge when presented with irrelevant context. In this work, we discover that, with proper prompting methods, instruction-finetuned LLMs can be highly controllable by contextual knowledge and robust to irrelevant context. Utilizing this feature, we propose EREN (Edit models by REading Notes) to improve the scalability and robustness of LLM editing. To better evaluate the robustness of model editors, we collect a new dataset, that contains irrelevant questions that are more challenging than the ones in existing datasets. Empirical results show that our method outperforms current state-of-the-art methods by a large margin. Unlike existing techniques, it can integrate knowledge from multiple edits, and correctly respond to syntactically similar but semantically unrelated inputs (and vice versa). The source code can be found at https://github.com/thunlp/EREN.

==> contents/problem.tex <==
\section{Sequential Model Editing}
\label{sec:model-editing-problem}

In model editing, multiple edits may be applied simultaneously or sequentially. The ability to perform the latter is important for making the edits as soon as they appear and has been shown to be considerably more challenging than the former scenario~\citep{t-patcher}. This paper focuses on sequential model editing.

When we apply one \textit{edit} $e$, we want to instill certain behaviors into a model $f$ on a set of inputs. Typically, $e$ is a fact and we want the edited model $f^*$ to behave as if the fact is true. The goal of model editing is to find an \textit{editor} function that produces an edited model given a \textit{base model} and an edit: $\text{Edit}(f, e) = f^*$.

To evaluate the correctness of $f^*$, we define the \textit{edit scope} $I(e)$ of $e$ as the set of input-output pairs that are implied by $e$:
\begin{equation*}
    I(e)=\{(x_1, y_1), ..., (x_m, y_m)\},
\end{equation*}
where $(x_i, y_i)$ is the $i$-th example implied by $e$.

For instance, the edit that instills the fact that ``The CEO of Apple is Tim Cook'' implies that the answer to the questions ``Who is the CEO of Apple?'' and ``Where does Tim Cook work?'' are ``Tim Cook'' and ``Apple'', respectively. 

% In a realistic scenario, multiple edits are applied online and sequentially.
In \textit{sequential} model editing, we want to apply each edit one by one and ensure that all intermediate edited models are performant. This is important for keeping the model up-to-date and undesired behaviors are fixed as soon as possible. Assume an ordered set of $n$ edits $\mathcal{E} = \{ e_1, ..., e_n \}$, the edited model is as follows.\footnote{$f_1 \circ f_2$ denotes the composite of $f_1$ and $f_2$.}
\begin{equation*}
\begin{small}
    f^* = \text{Edit}(f, \mathcal E) = \text{Edit}_n \circ \dots \circ \text{Edit}_2 \circ \text{Edit}_1 (f),
\end{small}
\end{equation*}
where $\text{Edit}_i(\cdot)=\text{Edit}(\cdot, e_i)$. Moreover, the edit scope of multiple edits is not the union of their scopes, because multiple edits in conjunction may imply new input-output pairs. Figure \ref{fig:framework} shows one such example in green. To address this, we denote the edit scope of a set of edits $I(\mathcal E)$ as all input-output pairs implied by all the edits in $\mathcal E$ in conjunction.%, and similarly for $O(\mathcal E)$.

The goal of $\text{Edit}(f,\mathcal {E})$ is to produce an $f^*$ that satisfies the following.
\begin{align*}
    f^*(x) = \begin{cases}
        y    & \forall(x, y) \in I(\mathcal E) \\
        f(x) & \forall x     \in \overline{I(\mathcal E)},
    \end{cases}
\end{align*}
where $\overline{\cdot}$ denotes the complement of a set.

For the simplicity of further discussion, we say an edit is \textit{relevant} to an input $x$ (and vice versa) when its edit scope contains $x$.

Note that the edits may come in different formats. Most existing works on model editing, represent edits with input-output pairs \cite{enn,mend,serac}, while others use factual triples \cite{rome,memit,remedi}. However, this paper assumes that edits are given as short declarative sentences. 
% We believe this is a more natural manner to "tell" the model the desired behavior because declarative sentences are the most common type of sentence.


\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{images/eren-framework3.pdf}
    \caption{Illustration of the framework of EREN. Two edits have been injected, and the colored part shows inference on two inputs. Green: Both edits are relevant, and the final output depends on both. Yellow: The reader determines that no edit is relevant, and the output of the base model is used.}
    \label{fig:framework}
\end{figure*}
